MUSIED: A Benchmark for Event Detection from Multi-Source Heterogeneous Informal Texts

Event detection (ED) identifies and classifies event triggers from unstructured texts, serving as a fundamental task for information extraction. Despite the remarkable progress achieved in the past several years, most research efforts focus on detecting events from formal texts (e.g., news articles, Wikipedia documents, financial announcements). Moreover, the texts in each dataset are either from a single source or multiple yet relatively homogeneous sources. With massive amounts of user-generated text accumulating on the Web and inside enterprises, identifying meaningful events in these informal texts, usually from multiple heterogeneous sources, has become a problem of significant practical value. As a pioneering exploration that expands event detection to the scenarios involving informal and heterogeneous texts, we propose a new large-scale Chinese event detection dataset based on user reviews, text conversations, and phone conversations in a leading e-commerce platform for food service. We carefully investigate the proposed dataset's textual informality and multi-source heterogeneity characteristics by inspecting data samples quantitatively and qualitatively. Extensive experiments with state-of-the-art event detection methods verify the unique challenges posed by these characteristics, indicating that multi-source informal event detection remains an open problem and requires further efforts. Our benchmark and code are released at \url{https://github.com/myeclipse/MUSIED}.

==> approach.tex <==
\section{Problem Formulation}
Different from most existing works, we formalize ED as a s Seq2Seq learning problem as follows. Let $S=$ ($w_{1},...,w_{n}$) be a sentence where $n$ is the sentence length and $w_i$ is the $i$-th token. Also, let $T=$ ($t_{1},...,t_{m}$) be the triggers within the sentence where $m$ is the number of triggers, and $y_i$ be the event type of $t_i$. An ED system needs to (1) map the sentence $S$ to a sequence of event type $Y=$ ($y_{1},...,y_{m}$), (2) locate the trigger $t_i$ for each generated event type $y_i$.

\section{The Proposed Approach}

\subsection{Overview}

We employ a classical attention-based encoder-decoder architecture for the problem defined above. As shown in Figure \ref{fig:overview}, the architecture consists of an encoder that converts the sentence $S$ into intermediate vectorized representation and a decoder that generates a sequence of event types. Further, we trace the triggers in encoder side for each generated event type, with the help of tracing attention mechanism.

The main characteristic of our architecture is that attention mechanism simultaneously plays two important roles: (1) help the decoder generate better label sequence by highlighting the important words just like classical attention mechanisms do, and (2) locate triggers for each generated event type, which is extremely important for our scenario. To balance these two objectives, we propose a novel attention mechanism, named \textbf{Tracing Attention}. Details of our method are introduced in the following.

\begin{figure}
    \centering
    \includegraphics[width=1.\linewidth]{figures/overview.png}
    \caption{The overall architecture of TSG. 
    The encoder projects the input sentence into hidden representation and the tracing attention based decoder generates event type sequence \{\emph{Die}, \emph{Attack}, \emph{Injure}\} sequentially. Further, the tracing attention is used to locate triggers. Note that locating process and the links from decoder cell to tracing attention layer are omitted for readability.}
    \label{fig:overview}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.5]{figures/overview.png}
%     \caption{The overall architecture of TSG. 
%     % The sentence contains \emph{Die}, \emph{Attack} and \emph{Injure} events triggered by ``killed'', ``fire'' and ``wounded'' respectively.
%     The encoder projects the input sentence into hidden representation and the tracing attention based decoder generates event type sequence \{\emph{Die}, \emph{Attack}, \emph{Injure}\} sequentially. Further, the tracing attention is used to locate triggers. Note that locating process and the links from decoder cell to tracing attention layer are omitted for readability.}
%     \label{fig:overview}
% \end{figure}

% The event detection task aims to extract the event types and their corresponding trigger words from the input sentence. Our hypothesis for this task is that the Seq2Seq-based paradigm can better capture the closeness among the event sequence and thus detect the events more accurately. Therefore, as shown in Figure \ref{fig:model}, We propose a novel  Seq2Seq-based paradigm for event detection, named Traceable Sequence Generation (TSG). The TSG mainly consists of two components: 1) a sentence encoder, which converts the input sentence into intermediate vectorized representations; and 2) an attention-based decoder, which generates the target event types according to the trigger words located by the tracing attention mechanism.

\subsection{Encoder}

Given a sentence $S=$ ($w_{1},...,w_{n}$), an encoder is adopted to encode the word sequence into a sequence of continuous representations $\vec{H}=(\vec{h}_1,...,\vec{h}_n)$. We use BERT followed by Bi-directional LSTM as encoder in the following:
% \footnote{Since we mainly explore the new paradigm, designing a sophisticated sentence encoder is not the scope of this paper.}:
\begin{equation}
\begin{aligned}
    \vec{\hat H} &= (\vec{\hat h}_1,...,\vec{\hat h}_n) = {\rm BERT}(w_{1},...,w_{n}) \\
    \vec{H} &=(\vec{h}_1,...,\vec{h}_n) = {\rm BiLSTM}(\vec{\hat h}_1,...,\vec{\hat h}_n)
\end{aligned}
\end{equation}
Following \citet{devlin:2018bert}, we append a ``[CLS]'' and ``[SEP]'' token to the head and tail of the input sentence.
% Since we mainly explore the new paradigm, a sophisticated sentence encoder is not the focus of this paper 


% Given a sentence of $n$ tokens ($w=w_0, ..., w_n$), sentence encoder is adapted to encode the sentence into sequence of hidden states $h=h_1, ..., h_n$. Since the main idea of our paper is to explore the effectiveness new paradigm based on Seq2Seq, and a sophisticated sentence encoder is not the focus of this paper. Therefore, we simply used the Bert and Bi-directional LSTM as our encoder to extract the semantics of the input sentence. 

% \begin{equation}
% \begin{aligned}
%     \hat h &= Bert(w_0, ..., w_n) \\
%     h &= BiLSTM(\hat h_0, ..., \hat h_n)
% \end{aligned}
% \end{equation}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1.\linewidth]{./figures/Attention.png}
    \caption{(a) Classical attention mechanism. (b) Our proposed tracing attention.}
    \label{fig:attention}
\end{figure}

\subsection {Tracing Attention}

Following \citet{liu2018exploiting}, we exploit supervised attention mechanism in this paper. For each decoding step, the ground-truth attention scores for trigger words are set to 1 while other words obtain 0.

Through preliminary investigation, we find training a decoder with classical supervised attention mechanism does not adequately drive the attention weights focusing on trigger words and some attention weights are still assigned to contextual words. It may be a reasonable phenomenon since contextual words do contribute to event types generation. However, diversified attention will inevitably hinder trigger word identification. Thus, we propose the tracing attention as Figure \ref{fig:attention} shows, which aims to force the decoder to depend solely on the most weighted word (or sub-word) when predicting an event type. This strategy is more consistent with the attention supervision signals (one-hot labels), achieving better collaboration between the objectives of generating labels and locating triggers.

% simply predicting an event type based on the classical supervised attention mechanism will not drive attention weights focusing on trigger words. 

% Even if we apply supervision signals to attention, some attention weights are still assigned to contextual words. 

% From the perspective of label generation, it is a reasonable phenomenon since contextual words do contribute to event types. However, diversified attention will inevitably hinder trigger word identification. Thus, we propose the tracing attention, which aims to force the decoder to depend solely on the most weighted word (or sub-word) when predicting an event type. This strategy is more consistent with the attention supervision signals (one-hot labels), achieving better collaboration between the objectives of generating labels and locating triggers. 





% To precisely locate event trigger, we propose the Tracing Attention which is supervised during training.
% Therefore, We design Tracing Attention to more precisely locate event triggers.
% Specifically, we force the decoder to depend solely on the most weighted word (or sub-word) when predicting an event type. This strategy is more consistent with the attention supervision signals (one-hot labels), achieving better collaboration between our two optimization objectives. Furthermore, we keep attention-related parameters from being updated by the generation objective during back-propagation. So that we can alleviate the dilemma that contextual words may compete for the attention weights of trigger words.



% Since the classical Seq2Seq model only focuses on generate output sequence effectively, how to efficiently locate the trigger words still remains a major challenge in the Seq2Seq-based event detection scenario. 

% The solve this problem, it is natural to exploit the attention mechanism to locate the trigger words. However, through preliminary investigation, we found simply predicting an event type based on the classical attention mechanism will not drive attention weights focusing on trigger words. Even if we apply supervision signals to attention, some attention weights are still assigned to contextual words. From the perspective of event classification, it is a reasonable phenomenon since contextual words do contribute to event types. However, diversified attention will inevitably hinder trigger word identification. 

% Therefore, We design a novel attention mechanism (named \textbf{Tracing Attention}) to precisely locate event triggers. Specifically, we force the decoder to depend only on the most weighted word (or sub-word) when predicting an event type. This strategy is more consistent with the attention supervision signals (one-hot labels), achieving better collaboration between our two optimization objectives. Furthermore, we keep attention-related parameters from being updated by the event classification objective during back-propagation. So that we can alleviate the dilemma that contextual words may compete for the attention weights of trigger words.

\subsubsection {Attention Calculation And Locating}

We use Luong attention and locate the most weighted word from the inputs sentence according to the calculated attention weights. Specifically, the attention mechanism assigns the preliminary weight $\hat \alpha_{ti}$ to the $i$-th word at time-step $t$ as follows:
\begin{equation}
    \hat \alpha_{ti} = \frac{{\rm exp}(\vec{s_t} \vec{W_a} \vec{h_i})}{\sum_{j=1}^{n} {\rm exp}(\vec{s_t} \vec{W_a} \vec{h_j})}
\end{equation}
where $\vec{W_a}$ is trainable parameter and $\vec{s_t}$ is the hidden state of the decoder at time-step $t$.
By traversing the attention scores, we locate the most-weighted word. Then the attention score is set to 1 for this word and 0 for others by a mask operation. The operation is shown in the following:
\begin{equation}
    \vec{\alpha_{t}} = \vec{I_t} \odot \vec{\hat \alpha_t}
\end{equation}
where $\vec{I_t}$ is a one-hot mask vector that is used to pick the most-weighted word and filter other words, $\odot$ is the element-wise production.




% \begin{equation}
% \begin{aligned}
%     % \hat s_t &= LSTM(s_{t-1}, \hat y_{t-1}) \\
%     \hat \alpha_{ti} &= exp(s_t W_{a} h_i) / \sum_{j=1}^{m} exp(s_t W_{a} h_j) \\
% \alpha_{ti} &= 
% \begin{cases}
% 	1 & if\ argmax(\hat \alpha_{t}) = i\\
% 	0 & otherwise
% \end{cases}
% \end{aligned}
% \end{equation}
% with $s = \{s_0, ..., s_m\}$ is the decoder variables for each time step in LSTM layer, $\hat y_{t-1}$ is the event type embedding predicted by last time step. 

\subsubsection {Dynamic Teacher Forcing Strategy}
At early stages of training, the insufficiently-trained attention mechanism  may inevitably cause error propagation and affect the training convergence. To tackle such issue, we propose to use teacher forcing strategy by picking the ground-truth trigger \footnote{If the trigger consists of multiple words, we select the most informative word which is usually a verb or noun. 
% For example, ``took office'' triggers an \emph{Start-Position} event and we select set attention score of ``took'' to 1.
} with the mask vector $\vec{I_t}$. Also, to alleviate the exposure bias problem, we 
exploit a dynamic teacher forcing strategy in this paper. Specifically, for each instance, we sample a binary value $m \in \{0,1\}$ from a Bernoulli($\rho$) distribution with high $\rho$ parameter and perform the following operation:
\begin{equation}
    \vec{I_t} = m \vec{I_t^{g}} + (1-m) \vec{I_t^{p}}
\end{equation}
where $\vec{I_t^g}$ denotes the constructed mask vector with ground-truth triggers while $\vec{I_t^p}$ denotes mask vector revealing the predicted most-weighted word. The final context vector $\vec{c_t}$ which is passed to decoder at time-step $t$ is calculated as:



% To accelerate convergence and reduce error accumulation especially at early stages of training, we exploit a dynamic teacher forcing for attention mechanism. More specifically, we sample instances from a Bernoulli distribution and set attention score of ground-truth trigger to 1 and filter other words \footnote{If the trigger consists of multiple words, we select the most informative word which usually is a verb. For example, ``took office'' triggers an \emph{Start-Position} event and we select set attention score of ``took'' to 1.}, while the rest samples keep the above calculated attention scores. The final context vector $\vec{c_t}$ which is passed to the decoder at time-step $t$ is calculated as follows:
\begin{equation}
    \vec{c_t} = \sum_{i=1}^n \alpha_{ti} \vec{h_i} 
\end{equation}

% Furthermore, inspired by the teacher forcing strategy in the Seq2Seq model, we proposed a teacher forcing attention strategy to accelerate convergence. More specifically, during training, we limited the most weighted word selection space from entire sentence to the ground truth trigger words with a certain probability, so that our model can effectively find the keyword. The teacher attention weights $\alpha_{t}^{teacher}$ can be computed as follows:

% \begin{equation}
% \begin{aligned}
%     \hat \alpha_{ti}^{teacher} &= \hat \alpha_{ti} \alpha^{gold}_{ti} \\
% 	\alpha_{ti}^{teacher} &= 
% 	\begin{cases}
% 		1 & if\ argmax(\hat \alpha_{t}^{teacher}) = i\\
% 		0 & otherwise
% 	\end{cases}
% \end{aligned}
% \end{equation}
% with $\alpha^{gold}_{t}$ is the gold attention weights constructed based on the ground truth trigger words. More specifically, $\alpha^{gold}_{ti}$ is 1 if the $i_{th}$ word is the trigger word and 0 otherwise.

\subsubsection {Supervised Attention Loss}
We use Kullback-Leibler divergence as the supervised attention objective, which is calculated as follows:
\begin{equation}
\begin{aligned}
    L_{Att} = \sum_{t=1}^m D_{KL} (\vec{\alpha^*_t}|\vec{\hat \alpha_{t}})
\end{aligned}
\end{equation}
where $D_{KL}(p|q)=\sum_{x} p(x) \frac{p(x)}{q(x)}$, $\vec{\alpha^*_t}$ is the gold attention at time-step $t$ and $\vec{\hat \alpha_{t}}$ is the preliminary attention weights.  

To alleviate the dilemma that contextual words may compete for the attention weights of trigger words, we keep attention-related parameters from being updated by the generation objective during back-propagation.

% Since the attention-related parameters were prevented from the event classification objective, we used Kullback-Leibler divergence as the supervised attention objective to optimize these parameters:

% \begin{equation}
% \begin{aligned}
%     loss_{att} = \sum_{t=0}^m D_{KL} (\alpha^{gold}_{t}|\hat \alpha_{t})
% \end{aligned}
% \end{equation}


\subsection {Decoder}
We use LSTM as decoder and calculate hidden state $\vec{s_{t}}$ at time-step $t$ as follows:
\begin{equation}
    \vec{s_t} = {\rm LSTM}(\vec{s_{t-1}},g(\vec{y_{t-1}}),\vec{c_{t-1}})
\end{equation}
where $\vec{y_{t-1}}$ denotes the probability distribution over label space at time-step $t$-1 and $g(\vec{y_{t-1}})$ denotes the label has the highest probability under the distribution $\vec{y_{t-1}}$. After obtaining hidden state $\vec{s_t}$ and context vector $\vec{c_t}$, we generate probability distribution at time-step $t$ as follows:
\begin{equation}
\begin{split}
\vec{o_{t}} = & \vec{W_d}[\vec{s_t};\vec{c_t}] \\
\vec{y_{t}} = & {\rm Softmax} (\vec{o_t})
\end{split}
\end{equation}
where $\vec{W_d}$ is weight parameter. Given the ground-truth label $y_t$ at time-step $t$, we use $p(y_t|y_{<t}, S)$ to denote the cross-entropy loss at time-step $t$ where $y_{<t}$ denotes the previously-generated event types.

The overall optimization objective is defined as:
\begin{equation}
    \begin{split}
    L_{Gen} & = -\sum_{S\in D}\sum_{y_t\in S} p(y_t|y_{<t}, S)
    \end{split}
\end{equation}

\subsubsection{Decoding Sequence Construction}
We construct decoding sequence by collecting event types of the triggers in a left-to-right manner as Figure \ref{fig:overview} shows and retain the duplicated labels. Each decoding sequence ends with \emph{EOS}. For sentences without events, we use a special label \emph{None} as the decoding target to help the model identify such sentences, and gold attention for this label concentrates on the tail word ``SEP'' of input sentence. We also explore other decoding sequence construction methods such as ``\emph{non-duplication-style}'', ``\emph{random-style}'' and ``\emph{sorted-style}'' in the experiments.
\subsubsection{Bag-of-Labels Constraint}
Instead of solely optimizing maximum likelihood estimation at each time-step, we also introduce a sentence-level bag-of-labels constraint as optimization objective, which penalizes out-of-bag prediction and award in-bag generation. 
We calculate the sentence-level probability of the generated bag-of-labels as follows:
\begin{equation}
    \vec{p_b} = {\rm \sigma} (\sum_{t=1}^m \vec{o_t}) 
\end{equation}
where $\vec{p_b}$ is a vector with length equal to label vocab size and represents how possible the label appears in the whole generated sequences. $\sigma$ denotes the $\rm Sigmoid$ function. We use Kullback-Leibler divergence as optimization objective, which is computed as follows:

\begin{equation}
\begin{aligned}
    L_{Bol} = \sum_{t=1}^m D_{KL} (\vec{\vec{p_b}^*}|\vec{p_b})
\end{aligned}
\end{equation}
where $\vec{\vec{p_b}^*}$ denotes the gold bag-of-label distribution which set the labels within the decoding target to 1 and others to 0.

\subsection{Training and Optimization}
TSG's overall optimization objective is defined as follows:
\begin{equation}
    J(\theta)  = L_{Gen} + \alpha L_{Att} + \beta L_{Bol} 
\end{equation}
where $\alpha$ and $\beta$ are weights for supervised attention loss and bag-of-labels constraint loss.
During training, we apply the teacher forcing mechanism where the gold label is used as input for each time-step, c paralleled computation and greatly accelerates the training process. We use dynamic teacher forcing strategy for the tracing attention.
Once the model is trained, we employ the beam search algorithm to find the top-ranked prediction path at inference time. 
The prediction paths ending with the \emph{EOS} are added to the candidate path set. 
Note that we perform a very simple data augmentation to meet the data volume requirement of the generative model. Specifically, we concatenate two original sentences and their corresponding event type sequences as the augmented data.

\subsection{Attention-Based Trigger Tracing}
After the event type sequence is generated, we locate trigger with the tracing attention scores. Though single-word triggers account for the vast majority (95.6\%), we noticed some multiple-word triggers in the dataset (4.4\%). We treat tokens with attention score larger than a threshold as candidate triggers and perform very simple post-processing. For example, since BERT uses WordPiece tokenization, we sum attention scores of the corresponding sub-tokens as the attention score for the word. We extract the contiguous sub-sequence with the highest probability from discontinuous tokens as multiple-word triggers. The threshold ranges from 0.1 to 0.5 with an interval of 0.1 and is tuned on the dev set.


% Finally, the total loss function for TSG is:

% \begin{equation}
% \begin{aligned}
% loss &= loss_{dec} + \alpha loss_{att} + \beta loss_{bag}
% \end{aligned}
% \end{equation}
% with $\alpha, \beta$ are weights of the attention loss and bag-of-words loss respectively.
